VAULT: VAriable Unified Long Text Representation for Machine Reading Comprehension

Existing models on Machine Reading Comprehension (MRC) require complex model architecture for effectively modeling long texts with paragraph representation and classification, thereby making inference computationally inefficient for production use. In this work, we propose VAULT: a light-weight and parallel-efficient paragraph representation for MRC based on contextualized representation from long document input, trained using a new Gaussian distribution-based objective that pays close attention to the partially correct instances that are close to the ground-truth. We validate our VAULT architecture showing experimental results on two benchmark MRC datasets that require long context modeling; one Wikipedia-based (Natural Questions (NQ)) and the other on TechNotes (TechQA). VAULT can achieve comparable performance on NQ with a state-of-the-art (SOTA) complex document modeling approach while being 16 times faster, demonstrating the efficiency of our proposed model. We also demonstrate that our model can also be effectively adapted to a completely different domain -- TechQA -- with large improvement over a model fine-tuned on a previously published large PLM.

==> VAULT Camera Ready/conclusions.tex <==
\section{Conclusions}
In this work we introduce and examine a powerful yet simple model for reading comprehension on long texts which we call \systemname, based on the hypothesis that with a large sequence length long answers can be classified effectively without computationally heavy graph-based models.  We validate our approach by showing it yields F1 scores competitive with heavier methods at a fraction of the decoding cost on two very different domain benchmark datasets that require reading long texts.

%In this work we introduce and examine a powerful yet simple model for reading comprehension on long texts which we call \systemname, based on the hypothesis that with a large sequence length long answers can be classified effectively without computationally heavy graph-based models.  We show that our approach yields F1 scores competitive with these heavier methods at a fraction of the decoding cost.  Further, we show that this approach generalizes to other datasets (TechQA).  


==> VAULT Camera Ready/experiments.tex <==
\section{Experiments}

% \subsection{Datasets}
\textbf{Datasets}: We experiment with two challenging ``natural'' MRC datasets: NQ \cite{kwiatkowski-etal-2019-natural} and TechQA \cite{Castelli-techqa-2020-acl}. We provide a brief summary of the datasets and direct interested readers to the corresponding papers.
%\avi{make the dataset descriptions much shorter Anthony e.g. one sentence for each this is a short paper.}
NQ consists of crowdsourced-annotated \textit{full} Wikipedia pages which appear in Google search logs with two tasks: the start and end offsets for the short answer (SA) and long answer (LA, eg. paragraph) -- if they exist.
%This consists of 307,373 training examples (question and passage pair), 7,830 development (dev) examples, and 7,842 hidden test examples (only accessible via leaderboard submission).  Questions are taken from Google search logs with Wikipedia passage results.  Crowdsourced workers annotate the start and end offsets for the short answer (SA) and select a long answer (LA, eg. paragraph) if they exist.  Model predictions are required to provide a confidence score which is used to predict whether an answer exists.  
% \noindent \textbf{
TechQA is developed from real user questions in the customer support domain where each question is accompanied  by  50  documents  -- at  most  one of which has an answer -- with answers significantly longer 
%\avi{Anthony mention the percentage here.}
(\textasciitilde 3-5x) than standard MRC datasets like SQuAD. We report official F1 scores for each dataset. %for both datasets.
% \anthony{NQ is EM F1 not token overlap}
% This consists 600 training queries, 310 development queries, and 490 hidden test queries (also only accesible through a leaderboard submission) from the technical support domain.  For each query 50 Technotes are provided, possibly containing an answer which are significantly longer \avi{Anthony mention the percentage here.} than standard MRC datasets like SQuAD.

% \noindent \textbf{Results on NQ}:
% We train the model described in section \ref{sec:models} on NQ and compare against Longformer and \dm using the base variants of all models implemented in the Huggingface toolkit\footnote{\url{https://github.com/huggingface/transformers}}.  Our Longformer baseline is implemented in the style of \cite{Alberti-bert-baseline-2019, pan-frustratingly-2019} where we first predict the SA and then select the enclosing LA.  We aim to show that our method provides an improvement over Longformer while being much cheaper to decode than \dm.  To do this we consider dev SA and LA F1 as well as decoding time $t_{decode}$ as evaluation metrics.

% In table \ref{tab:NQ} we report the results on NQ.  Adding classifcation of HTML tags gives an improvement of 2 LA F1 points at the cost of 0.4 SA F1 and 19m of decoding time.  LA F1 is improved by directly predicting the LA first before then selecting the SA, as opposed to selecting the best SA first and then choosing the enclosing LA.  As a consequence of this there is a small decrease in SA F1.  The additional runtime usage similarly comes from classifying the LAs.  Our final \systemname model\footnote{Hyperparameters for final model: sequence length 4096, doc stride 2048 \cite{Ainslie-ETC-2020}, subsampling rates (no answer/has answer) 0.02/0.08, learning rate 5e-5, 4 epochs of training.} provides an additional 2.5 SA F1 and 2.8 LA F1 by adding GPO; thus showing the benefit of giving partial credit to nearly correct positions.  As this is done at training there is no increase to decoding time.  \systemname is competitive with \dm in F1 score at 0.6 worse on SA F1 and 0.3 better on LA F1.  
% %The downside of \dm is in its decoding time of 11h.  Our \systemname decodes over 10x quicker at only 40
% However when it comes to decoding time there is no contest: \systemname decodes over 16 times faster.

% \begin{table}[h]
% \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|cc|c}
% \hline
%   \textbf{Model} & \textbf{SA F1} & \textbf{LA F1} &  $\boldsymbol{t_\text{decode}}$  \\
%   \hline
%   \dm & \textbf{52.2} & 70.1 & 11h   \\
% \hline
%   Longformer  & 49.5 & 65.6 & \textbf{22m} \\
% \hline
%   + Classify HTML Tag & 49.1 & 67.6  & 41m \\
% %\hline
%   + GPO (\systemname) & 51.6  & \textbf{70.4} & 40m   \\
%   \hline
% \end{tabular}%
% }
% \caption{Results on NQ dev set.}
%   \label{tab:NQ}
% \end{table}
\noindent \textbf{Results on NQ}: We train \systemname{} on NQ -- predicting the paragraph and span answers as NQ's LA and SA respectively -- and compare against \dm{}: a RoBERTa \cite{liu-roberta-2019} variant of the SOTA document model (DM) \cite{zheng-etal-2020-document-acl} 
% Anthony: removing to reword to SOTA
% and our main competitor (we both use paragraph representation to improve LA performance)
%\heng{what do you mean by 'our main competitor?}
using the base variants
% implemented in the Huggingface toolkit\footnote{\url{https://github.com/huggingface/transformers}}
for a more systematic comparison.  Although it may seem fair to include a Longformer DM baseline in our table, doing so would be infeasible (and unwise) due to production resource constraints.
We further show the impact of \systemname{} by providing ablation experiments where its components (GPO and PAPR) are removed.  The base LM (Longformer in our experiments) without GPO and PAPR, is implemented in the style of \cite{Alberti-bert-baseline-2019,NQ_COLING} where we first predict the SA and then select the enclosing LA.  We aim to show that our proposed method provides comparable results to \dm{} while being considerably faster while decoding and displaying improved performance over experiments just using the language model.  To do this we consider development set SA and LA F1 (the F1 metrics with respect to the span and paragraph answers respectively)
%\heng{explain these metrics} 
as well as decoding time $t_\text{decode}$ (on a V100) as metrics.
%  We further show the impact of \systemname by providing ablation experiments where its components (GPO and HTML tag classification) are removed.  Our baseline without LA (HTML tag) classification is implemented in the style of \cite{Alberti-bert-baseline-2019, pan-frustratingly-2019} where we first predict the SA and then select the enclosing LA.  We aim to show that our method provides comparable results to \dm while being much cheaper to decode and further provides improved performance over experiments with its components removed.  To do this we consider dev SA and LA F1 as well as decoding time $t_{decode}$ as evaluation metrics.

Table \ref{tab:NQ} shows the results on the NQ dev set.  We see \systemname{} and \dm{}  provide comparable F1 performance (precision and recall are shown in the Appendix). However, when it comes to decoding time, we can find \systemname{} decodes over 16 times faster than \dm{}. We additionally see in the ablation experiments that our enhancements increase both F1 metrics by multiple points, at the expense of some decoding time.  In particular we note that the F1 performance of Longformer is not competitive with \systemname{}.  We conclude that \systemname{} provides the best balance of F1 and decoding time as it is effectively tied on F1 (with \dm{}) and is only around 20 minutes slower to decode than the quickest model.

% In Table \ref{tab:NQ} we report the results on the NQ dev set.
% We see \systemname and \dm  provide comparable performance at 0.6 worse on SA F1 and 0.3 better on LA F1. However when it comes to decoding time there is no contest: \systemname decodes over 16 times faster showing a big improvement!
% \avi{I need to spend 2 more hrs to finish up : I'm thinking of calling this classify html tags as EPR: enhanced paragraph representation. Once we agree I'll modify section 3.1 and then also this. }
% Further, we empirically show the improvement made by \systemname.  When removing the partial credit of GPO, 2.5 SA F1 and 2.8 LA F1 is lost.  As this is implemented at training there is effectively no change in decoding time.  Further removing the classification of HTML tags -- and no longer directly predicting the LA first before then selecting the SA -- sees an additional decrease in performance of 2 LA F1, a gain of 0.4 SA F1, and decoding approximately 20 minutes quicker.  The small gain in SA F1 is due to selecting the best SA first and then choosing the enclosing LA.  The decoding speedup comes from not ``classifying" LAs at all and just selecting them.  Overall, \systemname provides a boost of 2.1 SA F1 and 4.8 LA F1 at the cost of only around 20 minutes of decoding time when compared to the model with its features removed. 
% \heng{all of these sentences in this paragraph are repeating some obvious results from the table. replace it with something more insightful}

\begin{table}[h]
\centering
\small
    \begin{tabular}{l|cc|c}
\hline
   \textbf{Model} & \textbf{SA F1} & \textbf{LA F1} &  $\boldsymbol{t_\text{decode}}$  \\
   \hline
  \dm & \textbf{52.2} & 70.1 & 11h   \\
\hline
   \systemname  & 51.6  & \textbf{70.4} & 40m \\
\hline
   - GPO & 49.1 & 67.6  & 41m \\
%\hline
   - PAPR (Longformer) & 49.5 & 65.6 & \textbf{22m}   \\
   \hline
\end{tabular}
\caption{Comparison of \systemname{} vs. \dm \ on NQ. We achieve comparable performance while being 16 times faster.}
  \label{tab:NQ}
\end{table}



% \begin{table}[h]
% \centering
% \small
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|cc|c}
% \hline
%   \textbf{Model} & \textbf{SA F1} & \textbf{LA F1} &  $\boldsymbol{t_\text{decode}}$  \\
%   \hline
%   \dm & \textbf{52.2} & 70.1 & 11h   \\
% \hline
%   \systemname  & 51.6  & \textbf{70.4} & 40m \\
% \hline
%   - GPO & 49.1 & 67.6  & 41m \\
% %\hline
%   - PAPR & 49.5 & 65.6 & \textbf{22m}   \\
%   \hline
% \end{tabular}%
% }
% \caption{Comparison of \systemname vs. \dm on NQ. We achieve comparable performance while being 16 times faster.}
%   \label{tab:NQ}
% \end{table}
% \heng{maybe should try to get further gains, and provide qualitative analysis}
% \anthony{We tried to get further gains and the best we were able to do in the time we had was match DM's performance.}


\noindent \textbf{Domain Adaptation: Results on TechQA}: Since \systemname{} has shown to be effective on NQ, we evaluate it on a new domain, TechQA.  We compare it against a RoBERTa base model trained with the same hyper-parameters as \cite{Castelli-techqa-2020-acl} -- except we use 11 epochs instead of 20.  We chose base instead of large (as is used for the TechQA baseline) to give a fair comparison since we are using a base PLM for our experiments with \systemname.  Similarly, we use RoBERTa rather than BERT as it is closer to Longformer. 
% \avi{All this base v. large justifications can be moved to the appendix thereby giving plenty of space. Also the Github link of TechQA etc can move to the appendix or just create a citation with the Github link.} \anthony{I can move it to the appendix, however seems like this risks comments from reviewers (they don't have to read appendix) complaining these results are not SOTA or matching something else so reject.  We can refer them to appendix then, do you think this is worth it for the space?} 
Having already established the run-time effectiveness of \systemname{} on NQ, we focus on F1 metrics here, including ``has answer'' (HA) F1.  We consider HA F1 our primary metric as we are exploring paragraph answer extraction in this work and (as previously mentioned) answers in TechQA are much longer than other datasets. %\anthony{@avi added sentence from slack message.}
We believe that the improvements in HA F1, at least partially, come from GPO.

\begin{table}[h]
\centering
\small
\begin{tabular}{l|cc}
\hline
 %\textbf{Model}& \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}} \\
 
   \textbf{Model} & \textbf{F1} & \textbf{HA F1} \\
   \hline
  RoBERTa & 48.6 & 7.6    \\
\hline
   \systemname & \textbf{49.3}  & \textbf{16.1}    \\
   \hline
\end{tabular}
\caption{Results on TechQA dev set. \systemname{} clearly outperforms RoBERTa on both F1 and Has Answer F1.}
  \label{tab:TechQA}
\end{table}

Results on TechQA are reported in Table \ref{tab:TechQA}.  We see that our \systemname{} model provides an improvement of 0.7 F1 and 8.5 HA F1 (denotes Has Answer); thus showing the effectiveness of our approach.  In particular, we see that this approach of imputing a paragraph structure to classify provides a large boost to performance when a non-null answer exists (HA F1).

==> VAULT Camera Ready/intro.tex <==
\section{Introduction}

Machine Reading Comprehension (MRC) has seen great advances in recent years with the rise of pre-trained language models (PLM) \cite{devlin-etal-2019-bert,liu-roberta-2019,lan2019albert} and public leaderboards \cite{Rajpurkar_2016,rajpurkar2018know,yang2018hotpotqa,joshi-etal-2017-triviaqa,welbl-etal-2018-wikihop,kwiatkowski-etal-2019-natural}.  While some challenges \cite{Rajpurkar_2016,rajpurkar2018know} focus on reading comprehension with shorter contexts, many others \cite{welbl-etal-2018-wikihop,joshi-etal-2017-triviaqa,kwiatkowski-etal-2019-natural,DBLP:journals/corr/abs-2101-11272} focus on longer contexts that cannot fit into a typical 512 sub-token transformer window.  Motivated by this, we focus on reading comprehension with long contexts.

One newer approach to this task \cite{zheng-etal-2020-document-acl} focuses on modeling document hierarchy to represent multi-grained information for answer extraction.  Although this approach creates a strong representation of the text, it suffers from a significant drawback. The graph-based methods \cite{velivckovic2018graph} are inefficient on parallel hardware, such as GPUs, resulting in slow inference speed \citep{zhou-2018-gnn,zheng-etal-2020-document-acl}.
Motivated by this, in this paper, we propose a reading comprehension model that addresses the above issue and uses a more light-weight, parallel-efficient (i.e. efficient on parallel hardware) paragraph representation based on long contextual representations for providing paragraph answers to questions. Instead of modeling document hierarchy from tokens to document pieces, we first introduce a base model that builds on top of a large ``long-context" PLM (we use Longformer, \citealp{beltagy-longformer-2020}) to model longer contexts with lightweight representations of each paragraph.  We note that while our approach could work with any PLM, we expect it to perform better with models that can support long contexts and therefore see more paragraph representations at once~\cite{gong-etal-2020-recurrent}.  To provide our model a notion of paragraph position relative to a text we also introduce position-aware paragraph representations (PAPR) utilizing special markup tokens and provide them as input for efficient paragraph classification.  This approach allows us to encode paragraph-level position in the text and teach the model to impute information on each paragraph into the hidden outputs for these tokens that we can exploit to determine in which paragraph the answer resides.  We then predict the answer span from this identified paragraph.

While previous MRC methods \cite{chen-etal-2017-reading,devlin-etal-2019-bert} use ground-truth start and end span positions exclusively as training objectives when extracting answer spans from the context and consider all other positions as incorrect instances equally. However, spans that overlap with the ground-truth should be considered as partially correct. Motivated by \citet{Li-gpo-2020-iclr} which proposes a new optimization criteria based on constructing prior distribution over synonyms for machine translation, we further propose to improve the above base model by considering the start and end positions of ground-truth answer spans as Gaussian-like distributions, instead of single points, and optimize our model using statistical distance.

We call this final model, \systemname{} (\textbf{VA}riable \textbf{U}nified \textbf{L}ong \textbf{T}ext representation) as it can handle a variable number and lengths of paragraphs at any position with the same unified model structure to handle long texts.

To evaluate the performance of \systemname, we select the new Natural Questions (NQ, \citealp{kwiatkowski-etal-2019-natural}) and TechQA \cite{Castelli-techqa-2020-acl} datasets.  NQ attempts to make Machine Reading Comprehension (MRC) more realistic by providing longer Wikipedia documents as contexts and real user search-engine queries as questions, and aims at avoiding \textit{observation bias}: high lexical overlap between the question and the answer context which can happen frequently if the question is created after the user sees the paragraph \cite{Rajpurkar_2016,rajpurkar2018know,yang2018hotpotqa,NQ_COLING,karpukhin-etal-2020-dense,lee2019latent,murdock_et_al_2018_engineered_ai}.
The task introduces the extraction of long answers (henceforth LA; typically paragraphs) besides also requiring short answers (henceforth SA) similar to SQuAD \cite{Rajpurkar_2016}.
%SAs are typically a span in LAs, though not formally required.
In Figure \ref{fig:examples} we examine an example from NQ along with the answers of \systemname{} and \cite{zheng-etal-2020-document-acl}.  We see that while \systemname{} can extract answers from the very bottom of a page -- if relevant -- the existing system suffers from positional bias.  It often predicts answers from the first paragraph of Wikipedia (a region which often contains the most relevant information).  
We evaluate our model for domain adaptation on TechQA, a recently introduced challenging dataset for QA on technical support articles where answers are typically 3-5 times longer 
than standard MRC datasets
\cite{Rajpurkar_2016,rajpurkar2018know}.
%Hence, we have one Wikipedia-based and one ``Tech-based" (different domain) evaluation datasets for \systemname{}.

\begin{figure}[ht]
     \fbox{\includegraphics[width=\columnwidth]{figs/vault.png}}
     \caption{Example from the NQ dataset with answers from \systemname{} and \cite{zheng-etal-2020-document-acl}.}
     \label{fig:examples}
%\vspace{-0.5cm} 
\end{figure}

Empirically we first show that \systemname{} achieves comparable performance on NQ with \cite{zheng-etal-2020-document-acl}'s document modeling architecture based on graph neural networks while being 16 times faster, demonstrating the efficiency of our proposed model.  Secondly, we show the generalization of our model architecture for domain adaptation on
%an entirely different-than-Wikipedia domain: 
TechQA.  Our experiments show that our model pre-trained on NQ can be effectively adapted to TechQA outperforming a standard fine-tuned model trained on a large PLM such as RoBERTa.
\noindent
To summarize, our contributions include:
% \heng{these are just experiment results, not 'contributions'. contributions need to highlight the new ideas. these bullets need to be re-written}

\begin{enumerate}\setlength\itemsep{-0.5mm}
    % \item We have developed an effective light-weight long context representation by modeling longer contexts.
    % \item We show that local contexts near ground-truth are more informative than irrelevant tokens and it is worthy to assign soft labels to such tokens while modeling long contexts. This model is called \systemname{}.
    % \item We show that these above techniques achieve competitive performance at par with more expensive SOTA models on NQ.
    % \item Finally, we showcase \systemname{}'s domain adaptation capability by putting it to test on an entirely new technical support domain for QA.
    \item We introduce a novel and effective yet simple paragraph representation.
    \item We introduce soft labels to leverage information from local contexts near ground-truth during training which is novel for MRC.
    \item Our model provides similar performance to a SOTA system on NQ while being 16 times faster and also effectively adapts to a new domain: TechQA.
    %\item Our model generalizes to domain adaptation on the TechQA challenge. \anthony{Added this too to bring more techqa to intro based on reviewer comment of NQ only, thinking it may need some refinement.  thoughts @hayoyang?}\haoyang{maybe we can merge 3 and 4 by emphasizing experiments are done in both NQ and TechQA?}
\end{enumerate}

==> VAULT Camera Ready/intro_old.tex <==
\section{Introduction}
%We discuss multiple strategies for MOdeling Long Documents... \\

% \heng{It's not clear what the novelty claims are in the introduction. Is the main novel point that you consider the position information of each paragraph? give some walk through example to show what's new and why it works, or point out the limitation of existing methods}
% \avi{Agree with you Heng. This is the weakest part of the paper right now. I'll work on this once I get a couple of good examples from Anthony.}

Question answering on long documents often involves modeling document hierarchy structures such as paragraphs. One of the example is the recently introduced \textit{Natural Questions} (NQ) dataset \cite{kwiatkowski-etal-2019-natural} attempts to make Machine Reading Comprehension (MRC) more realistic by providing longer Wikipedia documents as contexts and real user search-engine queries as the questions, and aims at avoiding \textit{observation bias}: high lexical overlap between the question and the answer context which can happen frequently if the question is created after the user sees the paragraph \cite{Rajpurkar_2016,rajpurkar2018know,yang2018hotpotqa,NQ_COLING,karpukhin-etal-2020-dense,lee2019latent,murdock_et_al_2018_engineered_ai} 
%\hans{Do we have a citation where obs. bias is shown on SQuAD?}.
% Machine reading comprehension (MRC), which requires systems to extract answers from a document given a question, has recently witnessed significant performance improvement on recent datasets \cite{Rajpurkar_2016,rajpurkar2018know, yang2018hotpotqa} due to the advent of large pre-trained language models (PLMs) \cite{devlin-etal-2019-bert,xlnet}. However, the recently introduced \textit{Natural Questions} (NQ) dataset \cite{kwiatkowski-etal-2019-natural} attempts to make MRC more challenging by providing longer Wikipedia documents as contexts and real user search-engine queries as the questions, avoiding \textit{observation bias}: high lexical overlap between the question and the answer context which can happen frequently if the question is created after the user sees the paragraph. 
The task also introduces the extraction of long answers (henceforth LA; typically a paragraph long) besides also requiring short answers (henceforth SA; similar to SQuAD \cite{Rajpurkar_2016}) SAs are typically a span in LAs, though not formally required.

\begin{figure}[ht]
     \fbox{\includegraphics[width=\columnwidth]{figs/vault.png}}
     \caption{Example from the NQ dataset.  See the Appendix for a VAULT overview figure.}
     \label{fig:examples}
%\vspace{-0.5cm} 
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \small
% \framebox{%
%   \begin{minipage}{\columnwidth}
%     \underline{\textbf{Example 1 (NQ)}} \\
% \textbf{Question:} when was the minimum wage established in the united states \\
% \textbf{Wikipedia Page:} Minimum Wage in the United States \\
% \textbf{Text:}
% The minimum wage in the United States is set by US labor law and a range of state and local laws. Employers generally have to pay workers the highest minimum wage prescribed by federal, state, and local law. Since \textcolor{hi-red}{July 24, 2009}, the federal government has mandated a nationwide minimum wage of \$7.25 per hour. [3] As of January 2018, there were 29 states with a minimum wage higher than the federal minimum. [4] From 2017 to 2018, eight states increased their minimum wage levels through automatic adjustments, while increases in eleven other states occurred through referendum or legislative action. [5] [6] Washington has the highest state minimum wage at \$11.50 per hour. [7] \\
% ... \\
% In 1933, the Roosevelt administration made the first attempt at establishing a national minimum wage, when a \$0.25 per hour standard was set as part of the National Industrial Recovery Act . However, in the 1935 court case Schechter Poultry Corp. v. United States (295 U.S. 495), the US Supreme Court declared the act unconstitutional, and the minimum wage was abolished. In \textcolor{hi-green}{1938}, the minimum wage was re-established pursuant to the Fair Labor Standards Act , once again at \$0.25 per hour (\$4.78 in 2017 dollars [28] ). In 1941, the Supreme Court upheld the Fair Labor Standards Act in United States v. Darby Lumber Co. , holding that Congress had the power under the Commerce Clause to regulate employment conditions. [29]  \\
%  ...
%   \end{minipage}}    
%   \caption{Examples question from the NQ dataset.  \systemname's correct short answer is shown in green,  incorrect baseline in red.  We note that the baseline incorrectly identifies the first paragraph, perhaps indicating a position bias in the model.  Please see the Appendix for more examples and discussion.
% %   \avi{Sorry Anthony on a second read these examples don't make much sense to me or are too complex for even NQ. Please send me some candidate ones and we can decide.}
%   }
%     \label{fig:examples}
% \end{figure}

Existing work on NQ typically involves extending pretrained language models (PLMs) \cite{Zaheer-bigbird-2020,Ainslie-ETC-2020,glass-etal-2020-span} and then applying a fine-tuning approach \cite{albert-synth-data,NQ_COLING} to predict SAs, then taking the surrounding paragraph as the LA. 
% \anthony{Mention RikiNet?  I removed it from this citation to focus on models which direct predict SA.}  
A significant shortcoming of such an approach is that when there is no SA it is not possible to predict an LA, as seen in Figure \ref{fig:examples} (these approaches predict the LA containing the SA). One newer approach \cite{zheng-etal-2020-document-acl} focuses on modeling document hierarchy to represent multi-grained information for answer extraction  and obtains SOTA on NQ -- directly predicting the LA and thereby overcoming this limitation. This approach suffers from a couple of drawbacks. First, the graph-based methods \cite{velivckovic2018graph} are inefficient on parallel hardware, such as GPUs, resulting in slow inference speed \citep{zhou-2018-gnn,zheng-etal-2020-document-acl}. 
% Attempts have also been made for modeling longer contextual information and have achieved impressive performance \cite{Ainslie-ETC-2020}\footnote{The code and model weights of ETC has not been released at the time of writing of the paper for us to have an accurate comparison.}.
Second, these approaches suffer from positional bias, as shown in Figure \ref{fig:examples} -- they often predict answers from the first paragraph of Wikipedia (a region which often contains the most relevant information).
In this paper, we propose a model that addresses the above issues and uses a more light-weight, parallel-efficient paragraph representation based on long contextual representations for providing long answers to questions. Instead of modeling document hierarchy from tokens to document pieces, we first introduce a base model that builds on top of a large ``long-context" PLM (we use Longformer \cite{beltagy-longformer-2020}) to model longer contexts with lightweight representations of each paragraph.  We note that while our approach could work with any PLM, we expect it to preform better with models that can support long contexts and therefore see more paragraph markup tokens at once.  To provide our model a notion of paragraph position relative to a Wikipedia page we also introduce position-aware paragraph representations utilizing special markup tokens and provide them as input for efficient long answer classification. Doing so, as shown in Figure \ref{fig:examples}, our model can extract answers from the very bottom of a page, if relevant;
%\anthony{added sents here to end of para for: ref to figure, more justification of PAPR, why we use longformer + that we could use something else}
we additionally show an overview of our model on this example in the Appendix.  This approach allows us to encode paragraph-level position in the document and teach the model to impute information on each paragraph into the hidden outputs for these tokens that we can exploit to determine in which paragraph the answer resides.  %\anthony{Remove rest of paragraph to save space?} Since various regions of a Wikipedia page can answer specific types of questions e.g. birthdays are usually in the first paragraph vs. spouse names are in the ``Personal Life'' paragraph, we model  paragraph representations within a page with special markup tokens and provide them as input for efficient long answer classification.
% We then directly use special paragraph tokens as representations for paragraph for long answer classification. \avi{this last sentence needs some work.}

% Performance on \textit{Natural Questions} has been boosted a lot by recent pretrain-model based neural architecture \cite{Zaheer-bigbird-2020,Ainslie-ETC-2020,liu-etal-2020-rikinet,glass-etal-2020-span,pan-frustratingly-2019}. Notably, One line of research focuses on modeling document hierarchy to represent multi-grained information for answer extraction \cite{zheng-etal-2020-document-acl}. However, the graph-based method is not efficient on parallel hardwares such as GPUs, which significantly affects prediction speed. Attempt has also been made for modeling longer contextual information and have achieved impressive performance \cite{Ainslie-ETC-2020}. In this paper, we proposed a model using more light-weighted and parallel-efficient paragraph  representations based on long contextual representations. Instead of modeling document hierarchy from tokens to document pieces, we first use Longformer \cite{beltagy-longformer-2020} to model longer contexts. Then we directly use special paragraph tokens as representations for paragraph for long answer classification.

While previous MRC methods \cite{chen-etal-2017-reading,devlin-etal-2019-bert} use ground-truth start and end span positions exclusively as training objectives when extracting answer spans from the context and consider all other positions as incorrect instances equally. However, spans that overlap with the ground-truth should be considered as partially correct. Motivated by \citet{Li-gpo-2020-iclr} which proposes a new optimization criteria based on constructing prior distribution over synonyms for machine translation, we further propose to improve the above base model by considering the start and end positions of ground-truth answer spans as Gaussian-like distributions, instead of single points. 
% \anthony{Remove this to save space?} These Gaussian-like distributions assign high probability mass on ground-truth positions, but they also assign soft probabilities to positions that are close to the ground-truth. Afterwards, we optimize the model based on these constructed priors. 
We call this final model, \systemname{} (\textbf{VA}riable \textbf{U}nified \textbf{L}ong \textbf{T}ext representation) as it can handle a variable number and lengths of paragraphs at any position with the same unified model structure to handle long texts.

% Besides, those span extraction based methods only use ground-truth start and end span positions as training objectives. However, spans that overlap with groundtruth should be considered as partially correct. Motivated by \citet{Li-gpo-2020-iclr} which proposes an new optimization based on prior distribution, we consider the start and end positions of groundtruth spans as Gaussian-like distributions, instead of single points. Those Gaussian-like distributions assign highest probability on groundtruth positions, but they also assign some probabilities to positions that are close to the groundtruth. Then we optimize the models based on those constructed priors.

Empirically we first show that \systemname{} achieves comparable performance on NQ with \cite{zheng-etal-2020-document-acl}'s document modeling architecture based on graph neural networks, while being more efficient. Secondly, we sow that our design decisions motivated by the NQ challenge are beneficial to other datasets by exploring the generalization of our model architecture for domain adaptation on an entirely different-than-Wikipedia domain: TechQA \cite{Castelli-techqa-2020-acl};
%\anthony{Added a bit here to say we make decisions based on NQ and then show generalization, thoughts @Haoyang?}
a recently introduced challenging dataset for QA on technical support articles where answers are typically 3-5 times  longer 
%\avi{Anthony please add stats from the TechQA ACL paper. You're an author there :) }
than standard MRC datasets %-- approximately 3-5x %other datasets
\cite{Rajpurkar_2016,rajpurkar2018know}. Our experiments show that our model pre-trained on NQ can be effectively adapted to TechQA outperforming a standard fine-tuned model trained on a large PLM such as RoBERTa.
% Experiments show that our proposed model has achieved comparable performance on Natural Questions with document modeling architecture based on graph neural networks, while our model is more efficient. Besides, we also explore the generalization of our model for domain adaptation on TechQA \cite{Castelli-techqa-2020-acl}. Our experiments shows that our model pretrained on Natural Questions can be effectively adapted to TechQA.
\noindent
To summarize, our contributions include:
% \heng{these are just experiment results, not 'contributions'. contributions need to highlight the new ideas. these bullets need to be re-written}

\begin{enumerate}\setlength\itemsep{-0.5mm}
    % \item We have developed an effective light-weight long context representation by modeling longer contexts.
    % \item We show that local contexts near ground-truth are more informative than irrelevant tokens and it is worthy to assign soft labels to such tokens while modeling long contexts. This model is called \systemname{}.
    % \item We show that these above techniques achieve competitive performance at par with more expensive SOTA models on NQ.
    % \item Finally, we showcase \systemname{}'s domain adaptation capability by putting it to test on an entirely new technical support domain for QA.
    \item We introduce a novel and effective yet simple paragraph representation.
    \item We introduce soft labels to leverage information from local contexts near ground-truth during training.
    \item Our model provides similar performance to a SOTA system on NQ while being computationally much faster and also effectively adapts to a new domain with better performance than SOTA models.
    \item Our model generalizes to domain adaptation on the TechQA challenge. \anthony{Added this too to bring more techqa to intro based on reviewer comment of NQ only, thinking it may need some refinement.  thoughts @hayoyang?}\haoyang{maybe we can merge 3 and 4 by emphasizing experiments are done in both NQ and TechQA?}
\end{enumerate}


==> VAULT Camera Ready/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> VAULT Camera Ready/models.tex <==
\section{Model Architecture}
\label{sec:models}

In this section, we introduce \systemname{}, our proposed model that uses a simple yet effective paragraph representation based on a longer context. \systemname{} starts from a base classifier that utilizes position-aware paragraph representations trained on top of a large PLM: Longformer \cite{beltagy-longformer-2020}. Next, we further introduce our Gaussian Prior-based training objective that considers partial credits for positions near the ground-truth, instead of only focusing on one ground-truth position. We show an overview of \systemname{} on the example from Figure \ref{fig:examples} in Figure \ref{fig:overview}.  

\begin{figure*}[ht]
    \centering
     \fbox{\includegraphics[width=\textwidth]{figs/overview.png}}
     \caption{Overview of \systemname{} answering the example from Figure~\ref{fig:examples}.  The 10th paragraph containing the correct answer is underlined.  The span linear layer receives hidden state outputs from all 4096 tokens in the window to create the start and end logits.  The paragraph linear layer receives the orange-highlighted [CLS] and markup tokens (e.g. [Para=10]) to predict in which paragraph the answer resides.  These logits are then used together to first select the best paragraph (LA) and finally select the best answer within said paragraph (SA).}
     \label{fig:overview}
\end{figure*}

% We show \systemname{} answering the same example from Figure \ref{fig:examples} in Figure \ref{fig:overview}.  
% A representation of the question and context (windowed) is formed with the paragraph tokens of PAPR imputed.  This input is then passed through the PLM to generate the hidden outputs.  PAPR then uses the hidden representations of these hidden tokens and the CLS token (to represent that there may not be any paragraph with the answer) -- highlighted in orange in the figure -- through a linear layer to produce paragraph logits (corresponding to LAs).  These logits are trained via maximum likelihood estimation (MLE).  For span answers (corresponding to SAs) we pass all tokens' hidden outputs through a linear layer to get start and end logits. These logits are trained with two objectives. One is the conventional MLE. Another is Gaussian Prior Objective, which optimizes the KL divergence between predicted distribution and constructed groundtruth distribution.

\subsection{A Base ``Paragraph'' Predictor Model}
SOTA methods for paragraph prediction \cite{zheng-etal-2020-document-acl, liu-etal-2020-rikinet} represent paragraphs through expensive graph modeling, making it inefficient for ``large-scale'' production MRC systems.  On the other hand, simply selecting the first paragraph performs poorly \cite{kwiatkowski-etal-2019-natural}. We hypothesize that by modeling a much longer context even simple paragraph representation can be effective for paragraph (i.e., long answers) classification. 
For this purpose, we employ a large-window PLM: Longformer \cite{beltagy-longformer-2020}, which has shown effectiveness in modeling long contexts for QA 
\cite{yang2018hotpotqa,welbl-etal-2018-wikihop,joshi-etal-2017-triviaqa}. Compared to conventional Transformer-based PLMs e.g. RoBERTa \cite{liu-roberta-2019} that can only take up to 512 sub-word tokens, Longformer provides a much larger maximum input length of 4,096. 

\noindent \textbf{Position-aware Paragraph Representation (PAPR)}: 
%Typically, since
To address the fact that many popular \textit{unstructured} texts such as Wikipedia pages
%are long and various regions of a Wikipedia page
%contain a mixture of structured specific 
have relatively standard ways of displaying 
% as where they represent 
%types of
certain relevant information (e.g. birthdays are usually in the first paragraph vs. spouse names are in the ``Personal Life'' paragraph), we provide the base model with a representation of which part of the text it is reading by marking the paragraphs with special atomic markup tokens (\texttt{[paragraph=i]}) at the beginning of each paragraph, indicating the position of the paragraph within the text\footnote{Similar tags are added for lists and tables.}.
With this input representation, we then directly perform long answer classification using the special paragraph token output embedding. Formally, for every paragraph $l_i \in P$, where $P$ are all paragraphs in a text and the representation for the corresponding markup token $\boldsymbol{h}^p_i$, the logit of a paragraph answer $a$ it computes is as $a^p_i = \boldsymbol{W}\boldsymbol{h}^p_i + \boldsymbol{b}$.

%\avi{is p a paragraph or tokens in a paragraph?}
% \[
% a^p_i = \boldsymbol{w_2}\textsc{Relu}(\boldsymbol{W}_1\boldsymbol{h}^p_i + \boldsymbol{b}_1 ) + b_2.
% \]
% \[
% a^p_i = \boldsymbol{W}\boldsymbol{h}^p_i + \boldsymbol{b}
% \]
% \anthony{Should this just be Wh + b?  I only do a single linear layer with no activation.}
We obtain additional document-piece representation from the standard \texttt{[CLS]} \cite{devlin-etal-2019-bert} token to model document pieces that do not contain paragraph answers. The probability of choosing the paragraph given context $\boldsymbol{c}$, is computed as the softmax over paragraph candidate (with an answer span) logits and not containing answer logit: 
\vspace{-1em}
% $p_l(l_i\mid \boldsymbol{c}) = \text{softmax}(a^p_i).$
\[
p_l(l_i\mid \boldsymbol{c}) = \text{softmax}(a^p_i).
\]
We pad the paragraph representations to ensure a rectangular tensor in a batch.
Our final prediction strategy is similar to \citet{zheng-etal-2020-document-acl} as we first choose the paragraph candidate with the highest logit among all candidates. We then extract span answers within the selected paragraph answer candidate using a standard pointer network.

\subsection{Gaussian Prior Optimization (GPO)}
Conventional span extraction models \cite{chen-etal-2017-reading, glass-etal-2020-span, liu-etal-2020-rikinet} optimize the probability of predicted start and end positions of the answer spans with ground-truth spans via maximum likelihood estimation (MLE,\citeauthor{wilks-1938-mle}, \citeyear{wilks-1938-mle}). MLE methods promote the probability for the ground-truth positions while suppressing the probability for all other positions. However we hypothesize that, for all those negative instances, the positions that are near the ground-truth should be given higher credit than farther distant positions, since the extracted answers will be partially overlapping with the ground-truth.

To tackle this problem, we follow the intuition from \citet{Li-gpo-2020-iclr} which proposes to promote the probability of generating synonyms using a Gaussian-like distribution for machine translation. We construct the distribution where it has the highest probability at ground-truth positions, and drop the probability exponentially as computed by the distance to the corresponding ground-truth positions. Specifically, for a groundtruth start or end position at $y_s$, where $s\in\{\text{start}, \text{end}\}$, we use a Gaussian distribution $\mathcal{N}(y_s, \sigma)$, where the mean is the position $y_s$ and variance $\sigma$ is a hyperparameter. We consider the probability density $\varphi(y\mid y_s, \sigma)$ of the Gaussian distribution at each position $y$ as the logit for the corresponding position. We then use the softmax function with temperature $T$ to re-scale the logits to get the Gaussian-like distribution $q(y\mid \hat{y}_s)$ for ground-truth distribution at position $y_s$, 
% $q(x\mid \hat{y}_s) = \text{softmax}(\varphi(x\mid \hat{y}_s, \sigma)/T).$
\[
q(y\mid y_s) = \text{softmax}(\varphi(y\mid y_s, \sigma)/T).
\]
We augment our MLE objective with an additional KL divergence \citep{kullback-1951-kld} term between constructed distribution $q(y\mid y_s)$ and model prediction $p_s(y\mid \boldsymbol{c}), s\in\{\text{start}, \text{end}\}$, so that we can guide our model to follow the Gaussian-like distribution for partial credit.
\begin{align*}
L_D \quad=\quad& KL\left(q(y\mid y_s)\parallel p_s(y\mid \boldsymbol{c}) \right) \\
\quad=\quad& \sum_y q(y\mid y_s)\log p_s(y\mid \boldsymbol{c})\\
-& \sum_y q(y\mid y_s)\log q(y\mid y_s).
\end{align*}
We refer to this final model as \systemname{}.

==> VAULT Camera Ready/related_work.tex <==
\section{Related Work}
Machine reading comprehension has been widely modeled as cloze-type span extraction \cite{chen-etal-2017-reading,cui_2017,devlin-etal-2019-bert}. In NQ, we need to identify answers in two levels, long and short answers. \cite{albert-synth-data} adapt a span extraction model for short answer extraction. \cite{zheng-etal-2020-document-acl,liu-etal-2020-rikinet} construct complex networks for paragraph-level representation to enhance long answer classification along with span extraction for short answers. In this work, we propose a more light-weight and parallel-efficient way for constructing paragraph-level representation and classification by using longer context and modeling the negative instance through Gaussian prior optimization.

Using the hierarchical nature of a long document for question answering has been previously studied by \cite{choi-etal-2017-coarse-to-fine-long-documents}, where they use a hierarchical approach to select candidate sentences and extract answers in those candidates. However, due to the limit of input length for large PLMs, existing methods \citep{Alberti-bert-baseline-2019,zheng-etal-2020-document-acl,NQ_COLING} slice long documents into document pieces and perform prediction for each piece separately. In our work, we show that by modeling longer input with position-aware paragraph representation coupled with Gaussian prior optimization (which is novel for MRC), we can achieve comparable performance using much simpler architecture compared to previous models, which coincide with recent new PLM for long inputs on question answering  \cite{Ainslie-ETC-2020}\footnote{The code and model weights of ETC has not been released at the time of writing of the paper for us to have an accurate comparison.}. 

==> VAULT Camera Ready/results.tex <==
\section{Results}

\subsection{NQ}

\subsection{TyDI QA}

==> intro_old.tex <==
\section{Introduction}
%We discuss multiple strategies for MOdeling Long Documents... \\

% \heng{It's not clear what the novelty claims are in the introduction. Is the main novel point that you consider the position information of each paragraph? give some walk through example to show what's new and why it works, or point out the limitation of existing methods}
% \avi{Agree with you Heng. This is the weakest part of the paper right now. I'll work on this once I get a couple of good examples from Anthony.}

Question answering on long documents often involves modeling document hierarchy structures such as paragraphs. One of the example is the recently introduced \textit{Natural Questions} (NQ) dataset \cite{kwiatkowski-etal-2019-natural} attempts to make Machine Reading Comprehension (MRC) more realistic by providing longer Wikipedia documents as contexts and real user search-engine queries as the questions, and aims at avoiding \textit{observation bias}: high lexical overlap between the question and the answer context which can happen frequently if the question is created after the user sees the paragraph \cite{Rajpurkar_2016,rajpurkar2018know,yang2018hotpotqa,NQ_COLING,karpukhin-etal-2020-dense,lee2019latent,murdock_et_al_2018_engineered_ai} 
%\hans{Do we have a citation where obs. bias is shown on SQuAD?}.
% Machine reading comprehension (MRC), which requires systems to extract answers from a document given a question, has recently witnessed significant performance improvement on recent datasets \cite{Rajpurkar_2016,rajpurkar2018know, yang2018hotpotqa} due to the advent of large pre-trained language models (PLMs) \cite{devlin-etal-2019-bert,xlnet}. However, the recently introduced \textit{Natural Questions} (NQ) dataset \cite{kwiatkowski-etal-2019-natural} attempts to make MRC more challenging by providing longer Wikipedia documents as contexts and real user search-engine queries as the questions, avoiding \textit{observation bias}: high lexical overlap between the question and the answer context which can happen frequently if the question is created after the user sees the paragraph. 
The task also introduces the extraction of long answers (henceforth LA; typically a paragraph long) besides also requiring short answers (henceforth SA; similar to SQuAD \cite{Rajpurkar_2016}) SAs are typically a span in LAs, though not formally required.

\begin{figure}[ht]
     \fbox{\includegraphics[width=\columnwidth]{figs/vault.png}}
     \caption{Example from the NQ dataset.  See the Appendix for a VAULT overview figure.}
     \label{fig:examples}
%\vspace{-0.5cm} 
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \small
% \framebox{%
%   \begin{minipage}{\columnwidth}
%     \underline{\textbf{Example 1 (NQ)}} \\
% \textbf{Question:} when was the minimum wage established in the united states \\
% \textbf{Wikipedia Page:} Minimum Wage in the United States \\
% \textbf{Text:}
% The minimum wage in the United States is set by US labor law and a range of state and local laws. Employers generally have to pay workers the highest minimum wage prescribed by federal, state, and local law. Since \textcolor{hi-red}{July 24, 2009}, the federal government has mandated a nationwide minimum wage of \$7.25 per hour. [3] As of January 2018, there were 29 states with a minimum wage higher than the federal minimum. [4] From 2017 to 2018, eight states increased their minimum wage levels through automatic adjustments, while increases in eleven other states occurred through referendum or legislative action. [5] [6] Washington has the highest state minimum wage at \$11.50 per hour. [7] \\
% ... \\
% In 1933, the Roosevelt administration made the first attempt at establishing a national minimum wage, when a \$0.25 per hour standard was set as part of the National Industrial Recovery Act . However, in the 1935 court case Schechter Poultry Corp. v. United States (295 U.S. 495), the US Supreme Court declared the act unconstitutional, and the minimum wage was abolished. In \textcolor{hi-green}{1938}, the minimum wage was re-established pursuant to the Fair Labor Standards Act , once again at \$0.25 per hour (\$4.78 in 2017 dollars [28] ). In 1941, the Supreme Court upheld the Fair Labor Standards Act in United States v. Darby Lumber Co. , holding that Congress had the power under the Commerce Clause to regulate employment conditions. [29]  \\
%  ...
%   \end{minipage}}    
%   \caption{Examples question from the NQ dataset.  \systemname's correct short answer is shown in green,  incorrect baseline in red.  We note that the baseline incorrectly identifies the first paragraph, perhaps indicating a position bias in the model.  Please see the Appendix for more examples and discussion.
% %   \avi{Sorry Anthony on a second read these examples don't make much sense to me or are too complex for even NQ. Please send me some candidate ones and we can decide.}
%   }
%     \label{fig:examples}
% \end{figure}

Existing work on NQ typically involves extending pretrained language models (PLMs) \cite{Zaheer-bigbird-2020,Ainslie-ETC-2020,glass-etal-2020-span} and then applying a fine-tuning approach \cite{albert-synth-data,NQ_COLING} to predict SAs, then taking the surrounding paragraph as the LA. 
% \anthony{Mention RikiNet?  I removed it from this citation to focus on models which direct predict SA.}  
A significant shortcoming of such an approach is that when there is no SA it is not possible to predict an LA, as seen in Figure \ref{fig:examples} (these approaches predict the LA containing the SA). One newer approach \cite{zheng-etal-2020-document-acl} focuses on modeling document hierarchy to represent multi-grained information for answer extraction  and obtains SOTA on NQ -- directly predicting the LA and thereby overcoming this limitation. This approach suffers from a couple of drawbacks. First, the graph-based methods \cite{velivckovic2018graph} are inefficient on parallel hardware, such as GPUs, resulting in slow inference speed \citep{zhou-2018-gnn,zheng-etal-2020-document-acl}. 
% Attempts have also been made for modeling longer contextual information and have achieved impressive performance \cite{Ainslie-ETC-2020}\footnote{The code and model weights of ETC has not been released at the time of writing of the paper for us to have an accurate comparison.}.
Second, these approaches suffer from positional bias, as shown in Figure \ref{fig:examples} -- they often predict answers from the first paragraph of Wikipedia (a region which often contains the most relevant information).
In this paper, we propose a model that addresses the above issues and uses a more light-weight, parallel-efficient paragraph representation based on long contextual representations for providing long answers to questions. Instead of modeling document hierarchy from tokens to document pieces, we first introduce a base model that builds on top of a large ``long-context" PLM (we use Longformer \cite{beltagy-longformer-2020}) to model longer contexts with lightweight representations of each paragraph.  We note that while our approach could work with any PLM, we expect it to preform better with models that can support long contexts and therefore see more paragraph markup tokens at once.  To provide our model a notion of paragraph position relative to a Wikipedia page we also introduce position-aware paragraph representations utilizing special markup tokens and provide them as input for efficient long answer classification. Doing so, as shown in Figure \ref{fig:examples}, our model can extract answers from the very bottom of a page, if relevant;
%\anthony{added sents here to end of para for: ref to figure, more justification of PAPR, why we use longformer + that we could use something else}
we additionally show an overview of our model on this example in the Appendix.  This approach allows us to encode paragraph-level position in the document and teach the model to impute information on each paragraph into the hidden outputs for these tokens that we can exploit to determine in which paragraph the answer resides.  %\anthony{Remove rest of paragraph to save space?} Since various regions of a Wikipedia page can answer specific types of questions e.g. birthdays are usually in the first paragraph vs. spouse names are in the ``Personal Life'' paragraph, we model  paragraph representations within a page with special markup tokens and provide them as input for efficient long answer classification.
% We then directly use special paragraph tokens as representations for paragraph for long answer classification. \avi{this last sentence needs some work.}

% Performance on \textit{Natural Questions} has been boosted a lot by recent pretrain-model based neural architecture \cite{Zaheer-bigbird-2020,Ainslie-ETC-2020,liu-etal-2020-rikinet,glass-etal-2020-span,pan-frustratingly-2019}. Notably, One line of research focuses on modeling document hierarchy to represent multi-grained information for answer extraction \cite{zheng-etal-2020-document-acl}. However, the graph-based method is not efficient on parallel hardwares such as GPUs, which significantly affects prediction speed. Attempt has also been made for modeling longer contextual information and have achieved impressive performance \cite{Ainslie-ETC-2020}. In this paper, we proposed a model using more light-weighted and parallel-efficient paragraph  representations based on long contextual representations. Instead of modeling document hierarchy from tokens to document pieces, we first use Longformer \cite{beltagy-longformer-2020} to model longer contexts. Then we directly use special paragraph tokens as representations for paragraph for long answer classification.

While previous MRC methods \cite{chen-etal-2017-reading,devlin-etal-2019-bert} use ground-truth start and end span positions exclusively as training objectives when extracting answer spans from the context and consider all other positions as incorrect instances equally. However, spans that overlap with the ground-truth should be considered as partially correct. Motivated by \citet{Li-gpo-2020-iclr} which proposes a new optimization criteria based on constructing prior distribution over synonyms for machine translation, we further propose to improve the above base model by considering the start and end positions of ground-truth answer spans as Gaussian-like distributions, instead of single points. 
% \anthony{Remove this to save space?} These Gaussian-like distributions assign high probability mass on ground-truth positions, but they also assign soft probabilities to positions that are close to the ground-truth. Afterwards, we optimize the model based on these constructed priors. 
We call this final model, \systemname{} (\textbf{VA}riable \textbf{U}nified \textbf{L}ong \textbf{T}ext representation) as it can handle a variable number and lengths of paragraphs at any position with the same unified model structure to handle long texts.

% Besides, those span extraction based methods only use ground-truth start and end span positions as training objectives. However, spans that overlap with groundtruth should be considered as partially correct. Motivated by \citet{Li-gpo-2020-iclr} which proposes an new optimization based on prior distribution, we consider the start and end positions of groundtruth spans as Gaussian-like distributions, instead of single points. Those Gaussian-like distributions assign highest probability on groundtruth positions, but they also assign some probabilities to positions that are close to the groundtruth. Then we optimize the models based on those constructed priors.

Empirically we first show that \systemname{} achieves comparable performance on NQ with \cite{zheng-etal-2020-document-acl}'s document modeling architecture based on graph neural networks, while being more efficient. Secondly, we sow that our design decisions motivated by the NQ challenge are beneficial to other datasets by exploring the generalization of our model architecture for domain adaptation on an entirely different-than-Wikipedia domain: TechQA \cite{Castelli-techqa-2020-acl};
%\anthony{Added a bit here to say we make decisions based on NQ and then show generalization, thoughts @Haoyang?}
a recently introduced challenging dataset for QA on technical support articles where answers are typically 3-5 times  longer 
%\avi{Anthony please add stats from the TechQA ACL paper. You're an author there :) }
than standard MRC datasets %-- approximately 3-5x %other datasets
\cite{Rajpurkar_2016,rajpurkar2018know}. Our experiments show that our model pre-trained on NQ can be effectively adapted to TechQA outperforming a standard fine-tuned model trained on a large PLM such as RoBERTa.
% Experiments show that our proposed model has achieved comparable performance on Natural Questions with document modeling architecture based on graph neural networks, while our model is more efficient. Besides, we also explore the generalization of our model for domain adaptation on TechQA \cite{Castelli-techqa-2020-acl}. Our experiments shows that our model pretrained on Natural Questions can be effectively adapted to TechQA.
\noindent
To summarize, our contributions include:
% \heng{these are just experiment results, not 'contributions'. contributions need to highlight the new ideas. these bullets need to be re-written}

\begin{enumerate}\setlength\itemsep{-0.5mm}
    % \item We have developed an effective light-weight long context representation by modeling longer contexts.
    % \item We show that local contexts near ground-truth are more informative than irrelevant tokens and it is worthy to assign soft labels to such tokens while modeling long contexts. This model is called \systemname{}.
    % \item We show that these above techniques achieve competitive performance at par with more expensive SOTA models on NQ.
    % \item Finally, we showcase \systemname{}'s domain adaptation capability by putting it to test on an entirely new technical support domain for QA.
    \item We introduce a novel and effective yet simple paragraph representation.
    \item We introduce soft labels to leverage information from local contexts near ground-truth during training.
    \item Our model provides similar performance to a SOTA system on NQ while being computationally much faster and also effectively adapts to a new domain with better performance than SOTA models.
    \item Our model generalizes to domain adaptation on the TechQA challenge. \anthony{Added this too to bring more techqa to intro based on reviewer comment of NQ only, thinking it may need some refinement.  thoughts @hayoyang?}\haoyang{maybe we can merge 3 and 4 by emphasizing experiments are done in both NQ and TechQA?}
\end{enumerate}


==> results.tex <==
\section{Results}

\subsection{NQ}

\subsection{TyDI QA}
